Morpho-kinematic properties of Wolf-Rayet planetary nebulae

The majority of planetary nebulae (PNe) show axisymmetric morphologies, whose causes are not well understood. In this work, we present spatially resolved kinematic observations of 14 Galactic PNe surrounding Wolf-Rayet ([WR]) and weak emission-line stars ($wels$) based on the H$\alpha$ and [N II] emission taken with the Wide Field Spectrograph on the Australian National University 2.3-m telescope. Velocity-resolved channel maps and position--velocity diagrams, together with archival Hubble Space Telescope ($HST$) and ground-based images, are employed to construct three-dimensional morpho-kinematic models of 12 objects using the program SHAPE. Our results indicate that these 12 PNe mostly have elliptical morphologies with either open or closed outer ends. The kinematic maps show the on-sky orientations of the interior shells in NGC6578 and NGC6629, as well as the compact ($\leq 6$ arcsec) PNe Pe1-1, M3-15, M1-25, Hen2-142, and NGC6567, in agreement with the elliptically symmetric morphologies seen in high-resolution $HST$ images. Point-symmetric knots in Hb4 exhibit deceleration with distance from the central star, which could be due to shock collisions with the ambient medium. The velocity dispersion maps of Pe1-1 also disclose the shock interaction between its collimated outflows and the interstellar medium. Collimated bipolar outflows are also visible in the position--velocity diagrams of M3-30, M1-32, and M3-15, which are reconstructed by tenuous prolate ellipsoids extending upward from dense equatorial regions in the kinematic models. The formation of aspherical morphologies and collimated outflows in these PNe could be related to the stellar evolution of hydrogen-deficient [WR] and $wels$ nuclei, which require further investigation.

==> figures1.tex <==

\figurenum{1}
\begin{figure*}
\begin{center}
%\plotone{figures/cel_diagnostic_diagram.eps}
\includegraphics[width=0.8\linewidth]{figure1/fig1_cel_dd_pb6.eps}\\
\includegraphics[width=0.8\linewidth]{figure1/fig1_cel_dd_m330.eps}\\
\caption{$N_{\rm e}$--$T_{\rm e}$ diagnostic diagrams based on CELs. The upper and lower limits at the 90\% confidence level are plotted by the dotted lines.  %}
\label{wc:fig:dd:cels:2}
%\figsetgrpstart
%\figsetgrpnum{1.1}
%\figsetgrptitle{image 1 caption}
%\figsetplot{figures/cel_diagnostic_diagram.eps}
%\figsetgrpnote{}
%\figsetgrpend
%\figsetend
%\newline
%(An extended version of this figure set is available in the online journal.) 
}
\end{center}
\end{figure*}

\figurenum{1}
\begin{figure*}
\begin{center}
\includegraphics[width=0.8\linewidth]{figure1/fig1_cel_dd_hb4shell.eps}\\
\includegraphics[width=0.8\linewidth]{figure1/fig1_cel_dd_hb4nknot.eps}\\
\caption{\textit{-- continued}}
\end{center}
\end{figure*}

\figurenum{1}
\begin{figure*}
\begin{center}
\includegraphics[width=0.8\linewidth]{figure1/fig1_cel_dd_ic1297.eps}\\
\includegraphics[width=0.8\linewidth]{figure1/fig1_cel_dd_th2a.eps}\\
\caption{\textit{-- continued}}
\end{center}
\end{figure*}

\figurenum{1}
\begin{figure*}
\begin{center}
\includegraphics[width=0.8\linewidth]{figure1/fig1_cel_dd_pe11.eps}\\
\includegraphics[width=0.8\linewidth]{figure1/fig1_cel_dd_m132.eps}\\
\caption{\textit{-- continued}}
\end{center}
\end{figure*}

\figurenum{1}
\begin{figure*}
\begin{center}
\includegraphics[width=0.8\linewidth]{figure1/fig1_cel_dd_m315.eps}\\
\includegraphics[width=0.8\linewidth]{figure1/fig1_cel_dd_m125.eps}\\
\caption{\textit{-- continued}}
\end{center}
\end{figure*}

\figurenum{1}
\begin{figure*}
\begin{center}
\includegraphics[width=0.8\linewidth]{figure1/fig1_cel_dd_hen2142.eps}\\
\includegraphics[width=0.8\linewidth]{figure1/fig1_cel_dd_hen31333.eps}\\
\caption{\textit{-- continued}}
\end{center}
\end{figure*}

\figurenum{1}
\begin{figure*}
\begin{center}
\includegraphics[width=0.8\linewidth]{figure1/fig1_cel_dd_hen2113.eps}\\
\includegraphics[width=0.8\linewidth]{figure1/fig1_cel_dd_k216.eps}\\
\caption{\textit{-- continued}}
\end{center}
\end{figure*}

\figurenum{1}
\begin{figure*}
\begin{center}
\includegraphics[width=0.8\linewidth]{figure1/fig1_cel_dd_ngc6578.eps}\\
\includegraphics[width=0.8\linewidth]{figure1/fig1_cel_dd_m242.eps}\\
\caption{\textit{-- continued}}
\end{center}
\end{figure*}

\figurenum{1}
\begin{figure*}
\begin{center}
\includegraphics[width=0.8\linewidth]{figure1/fig1_cel_dd_ngc6567.eps}\\
\includegraphics[width=0.8\linewidth]{figure1/fig1_cel_dd_ngc6629.eps}\\
\caption{\textit{-- continued}}
\end{center}
\end{figure*}

\figurenum{1}
\begin{figure*}
\begin{center}
\includegraphics[width=0.8\linewidth]{figure1/fig1_cel_dd_sa3107.eps}\\
\caption{\textit{-- continued}}
\end{center}
\end{figure*}



==> figures3.tex <==

\figurenum{3}
\begin{figure*}
\begin{center}
%\plotone{figures/cel_diagnostic_diagram.eps}
\includegraphics[width=0.325\linewidth]{figure3/fig3_pb6_n_ii_final.eps}
\includegraphics[width=0.325\linewidth]{figure3/fig3_m330_n_ii_final.eps}\\
\includegraphics[width=0.325\linewidth]{figure3/fig3_hb4shell_o_ii_final.eps}
\includegraphics[width=0.325\linewidth]{figure3/fig3_hb4shell_n_ii_final.eps}\\
\includegraphics[width=0.325\linewidth]{figure3/fig3_ic1297_c_ii_final.eps}
\includegraphics[width=0.325\linewidth]{figure3/fig3_ic1297_o_ii_final.eps}%
\includegraphics[width=0.325\linewidth]{figure3/fig3_ic1297_n_ii_final.eps}\\
\includegraphics[width=0.325\linewidth]{figure3/fig3_th2a_n_ii_final.eps}%\\\
\includegraphics[width=0.325\linewidth]{figure3/fig3_pe11_c_ii_final.eps}%
\includegraphics[width=0.325\linewidth]{figure3/fig3_pe11_n_ii_final.eps}\\
\caption{$T_{\rm e}$ diagnostic diagrams based on C\,{\sc ii} ORLs, and $N_{\rm e}$--$T_{\rm e}$ diagnostic diagrams based on O\,{\sc ii} and N\,{\sc ii} ORLs. %}
\label{wc:fig:dd:orls:2}
}
\end{center}
\end{figure*}

\figurenum{3}
\begin{figure*}
\begin{center}
\includegraphics[width=0.325\linewidth]{figure3/fig3_m132_c_ii_final.eps}%
\includegraphics[width=0.325\linewidth]{figure3/fig3_m132_n_ii_final.eps}
\includegraphics[width=0.325\linewidth]{figure3/fig3_m315_n_ii_final.eps}\\
\includegraphics[width=0.325\linewidth]{figure3/fig3_ngc6578_c_ii_final.eps}%
\includegraphics[width=0.325\linewidth]{figure3/fig3_ngc6578_o_ii_final.eps}%
\includegraphics[width=0.325\linewidth]{figure3/fig3_ngc6578_n_ii_final.eps}\\
\includegraphics[width=0.325\linewidth]{figure3/fig3_m242_c_ii_final.eps}%
\includegraphics[width=0.325\linewidth]{figure3/fig3_m242_o_ii_final.eps}%
\includegraphics[width=0.325\linewidth]{figure3/fig3_m242_n_ii_final.eps}\\
\includegraphics[width=0.325\linewidth]{figure3/fig3_ngc6567_c_ii_final.eps}
\includegraphics[width=0.325\linewidth]{figure3/fig3_sa3107_c_ii_final.eps}%
\caption{\textit{-- continued}}
\end{center}
\end{figure*}



